AutoModel: Automatic Synthesis of Models from Communication Traces of SoC Designs

Modeling system-level behaviors of intricate System-on-Chip (SoC) designs is crucial for design analysis, testing, and validation. However, the complexity and volume of SoC traces pose significant challenges in this task. This paper proposes an approach to automatically infer concise and abstract models from SoC communication traces, capturing the system-level protocols that govern message exchange and coordination between design blocks for various system functions. This approach, referred to as model synthesis, constructs a causality graph with annotations obtained from the SoC traces. The annotated causality graph represents all potential causality relations among messages under consideration. Next, a constraint satisfaction problem is formulated from the causality graph, which is then solved by a satisfiability modulo theories (SMT) solver to find satisfying solutions. Finally, finite state models are extracted from the generated solutions, which can be used to explain and understand the input traces. The proposed approach is validated through experiments using synthetic traces obtained from simulating a transaction-level model of a multicore SoC design and traces collected from running real programs on a realistic multicore SoC modeled with gem5.

==> src-cover-page.tex <==
% \noindent This table will be turned into a cover letter and be included in the TCAD reviewers.\\ \\
\noindent To,\\
Editor-in-Chief,\\
IEEE TRANSACTIONS ON COMPUTER-AIDED DESIGN OF INTEGRATED CIRCUITS AND SYSTEMS\\ \\
Respected Editor-in-Chief: \\
We are submitting our manuscript titled "{\sf AutoModel}: Automatic Synthesis of Models from Communication Traces of SoC Designs", an original contribution for consideration as a full-length journal paper in IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems (TCAD).

This work proposes a novel framework for synthesizing Finite State Automata models from concurrent System-on-Chip (SoC) execution traces. The extracted models are designed to aid in the discovery of system execution behavior, which is crucial for effective SoC debugging and testing. We want to highlight that this manuscript represents a substantial extension, comprising 70\% additional works, building upon our initial work published in ICCD 2021 [1]. The key ideas proposed in this paper are as follows:

· Model Synthesis from multiple traces (10\%) – The model synthesis Algorithm 1 [1], originally applied to a single trace, is extended to process a set of traces. By considering all input traces, the final inferred model becomes consistent with the entire set of traces.

· Trace Slicing on Message Attributes (10\%) –  We explore the use of micro-architecture attributes found in the traces to improve message correlation and more accurately calculate edge support for causality graphs in complex SoCs. It is discussed in Section VI-B.

· FSA-Based Model Evaluation Method (20\%) – This manuscript proposes a new evaluation approach called the \emph{acceptance ratio} (AR) to assess the quality of inferred models from input traces. The evaluation algorithm is a new contribution presented in Section VII.

· Comprehensive Experiments (20\%) – In this extension, we extensively validate our proposed method on various realistic SoC traces. This includes model synthesis from traces collected while booting a Linux kernel on a gem5 simulation model. The experimental results and findings are presented in sections VIII-A, VIII-B, VIII-C (1 - 2), and VIII-D of this paper. 

· Usage case study (10\%) – Section VIII-F presents a comprehensive usage case study demonstrating the protocol verification of gem5 simulation.\\


\noindent The corresponding author:\\
Md Rubel Ahmed\\
Dept. of Computer Sci. and Eng.\\
U of South Florida,\\
Tampa, FL\\ \\
The excluded associate editor:\\
Dr. Hao Zheng\\
U of South Florida,\\
Tampa, FL\\ \\
Thanks for your time. We look forward to hearing from you. \\
Sincerely,\\
Authors. \\

\noindent References  \\
$[\, 1 ]\,$ H. Zheng, M. R. Ahmed, P. Mukherjee, M. C. Ketkar and J. Yang, "Model Synthesis for Communication Traces of System Designs," 2021 IEEE 39th International Conference on Computer Design (ICCD), Storrs, CT, USA, 2021, pp. 492-499, doi: 10.1109/ICCD53106.2021.00082.

\begin{comment}
\begin{table*}[ht!]
\renewcommand{\arraystretch}{1.3}
\caption{Contribution on top of ICCD paper.}
\label{tab:tool_feature}
\centering
\begin{tabular}{|p{1.2in}|p{1.50in}|p{2.42in}|p{1in}|}
\hline
\multicolumn{1}{|c|}{Item} & \multicolumn{1}{c|}{ICCD}                                                                                                           & \multicolumn{1}{c|}{TCAD}                                                                                                                                                                                                                                                                                & Status \\ \hline
Literature                 & Short   & Detailed, more structured &        \\ \hline

Single vs multi CAS graph                 &   single graph & Multi-> single or many single to multi &  DONE      \\ \hline

Address Translation                 & No address translation                                                                                                                             & why and how to address translation is done for address slicing      &        \\ \hline
Multiple traces                 & Consider only one trace for Causality graph    & explain how to build causality graphs from multiple traces  & Done        \\ \hline
Slicing                 & Not Described                                                                                                                     & explain why/how packet id and address slicing differ.    & DONE        \\ \hline
Optimization               & Discussed windowing                                                                                                                 & \begin{tabular}[c]{@{}l@{}}Describes scopes of optimization, \\  1. Windowing is described in large\\  2. Trace Slicing based on:\\       a. Memory address slicing\\       b. Packet attribute slicing\\
3. Essential causality extraction
\end{tabular}                                                                                                                & DONE    \\ \hline
Experiments                & \begin{tabular}[c]{@{}l@{}}On synthetic and gem5\\   1. SE traces only \\   2. not comprehensive\\   3. Only one table\end{tabular} & \begin{tabular}[c]{@{}l@{}}Comprehensive Experiments\\ Discussion on gem5 trace generation\\ \st{1. Comparison with LSTM, T2M}\\     \st{Synoptic, FlowMiner (?)}\\ 2.  \st{Fault injection and faulty trace\\      detection.} \\ 3. \st{Evaluation Metrics like TPR,}\\      \st{TNR, precision and recall are}\\      \st{broadly described.}\end{tabular} &        \\ \hline
\end{tabular}
\end{table*}

\end{comment}
